Energy-Based Reranking: Improving Neural Machine Translation Using Energy-Based Models

The discrepancy between maximum likelihood estimation (MLE) and task measures such as BLEU score has been studied before for autoregressive neural machine translation (NMT) and resulted in alternative training algorithms (Ranzato et al., 2016; Norouzi et al., 2016; Shen et al., 2016; Wu et al., 2018). However, MLE training remains the de facto approach for autoregressive NMT because of its computational efficiency and stability. Despite this mismatch between the training objective and task measure, we notice that the samples drawn from an MLE-based trained NMT support the desired distribution -- there are samples with much higher BLEU score comparing to the beam decoding output. To benefit from this observation, we train an energy-based model to mimic the behavior of the task measure (i.e., the energy-based model assigns lower energy to samples with higher BLEU score), which is resulted in a re-ranking algorithm based on the samples drawn from NMT: energy-based re-ranking (EBR). We use both marginal energy models (over target sentence) and joint energy models (over both source and target sentences). Our EBR with the joint energy model consistently improves the performance of the Transformer-based NMT: +4 BLEU points on IWSLT'14 German-English, +3.0 BELU points on Sinhala-English, +1.2 BLEU on WMT'16 English-German tasks.

==> model_architecture.tex <==
% In this section, we will describe the architecture of our baseline NMT models and the EBM models. 
% \subsection{Base NMTs} \label{app:base}
% We use the Transformer \cite{vaswani&al17} implementation in Opennmt~\cite{opennmt} and Fairseq~\cite{ott2019fairseq} toolkits. 

% Our Transformer architecture include six encoder and six decoder layers, and the number of attention heads, embedding dimension and inner-layer dimension are 8, 512
% and 4096, respectively. We use dropout, weight decay, label smoothing to regularize our models. We use layer normalization and early stopping. Models are optimized using Adam~\cite{kingma2014method} with parameters $\beta_1 = 0.9$, $\beta_2 = 0.98$, and $\epsilon = 1e^{-8}$ and we use the same learning rate scheduler as \citeauthor{ott2019fairseq}~(\citeyear{ott2019fairseq}). We trained our models on 4 Nvidia TITANX GPUs.

% % \subsection{EBR architecture} \label{app:ebm}
% % To construct the energy network, we use a pretrained BERT~\cite{devlin-etal-2019-bert} from Huggingface~\cite{Wolf2019HuggingFacesTS} as our pretrained language model and project the mean-pooled hidden state of BERT into a scalar value. We use the \textit{BERT-base uncased} model with 12 encoder layers, 768 hidden state dimension, 12 attention heads and 110M parameters. For the projection, we use a 2-layer MLP with 256 hidden variables. In our experiments, we only train the parameters of the projection layer and the rest of BERT's parameters remain frozen. 



% % % the energy of samples generated from base NMT models are computed by projecting the samples down to a single scalar value. This is achieved by a architecture including a pretrained language model (LM) and a projection layer. We use a pretrained BERT \cite{devlin-etal-2019-bert} from Huggingface \cite{Wolf2019HuggingFacesTS} as our pretrained language model, as preliminary experiments have shown that it performed better. The sample hypothesis is fed to the pretrained BERT model. The projection layers takes the mean-pooled hidden state of BERT and converts it into a scalar. 

 
% % % The margin is calculated as \textit{margin(t, u) = BLEU(t, u)} \cite{10.3115/1073083.1073135}, where t is the target sequence and u is the sample sequence. The margin loss is formulated as : 
% % % \begin{align}
% % %     \mathcal{L}=\sum_{u} max[0, f(u, \theta) - f(t, \theta) + margin(t, u)]
% % % \end{align}
% % % Where $f(x, \theta)$ is the projection scalar for a sequence x and model parameter $\theta$. 

% % We use margin weight of $\alpha=10$ and temperature $T=1000$ for our experiments. We regularize the projection layer using L2 regularization.  Models are optimized using Adam \cite{kingma2014method} with parameters $\beta_1 = 0.9$, $\beta_2 = 0.98$, and $\epsilon = 1e^{-8}$ and a learning rate of $0.01$. 
% % % We train the projection layer parameters both individually and in shared methodology. This will be discussed in more details in the training setup section.
% % % During decoding, we rank our samples based on the  scalar score  generated  by  the  LM and projection layer and infer the  sample  with  highest  score  as EBM generated translation.
% % We run all experiments on 1 Nvidia TESLA M40 GPU.

% % % Additionally, we use L2 regularization on the projection output scalar to ensure that the projection output remains comparable to BLEU scores.

% \subsection{Language Models}\label{app:lm}
% In our BaseNMT+LM baseline, we use pretrained language model to calculate $\log P_{LM}(\mbf{y})$. For the \{De, Fr, It, Ro, Si, Ne\}$\xrightarrow{}$En tasks, we use a pretrained Transformer-XL~\cite{DBLP:journals/corr/abs-1901-02860} \textit{transfo-xl-wt103} and for the En$\xrightarrow{}$De task we use a pretrained XLM ~\cite{DBLP:journals/corr/abs-1901-07291} \textit{xlm-mlm-ende-1024}
% from Huggingface~\cite{Wolf2019HuggingFacesTS}.
